BlockMeter: An Application Agnostic Performance Measurement Framework For Private Blockchain Platforms

Blockchain Technology is an emerging technology with the potential to disrupt a number of application domains. Though blockchain platforms like Bitcoin and Ethereum have seen immense success and acceptability, their nature of being public and anonymous make them unsuitable for many enterprise level use-cases. To address this issue, Linux Foundation has started an open source umbrella initiative, known as the Hyperledger Platforms. Under this initiative, a number of private blockchain platforms have been developed which can be used for different enterprise level applications. However, the scalability and performance of these private blockchains must be examined to understand their suitability for different use-cases. Recent researches and projects on performance benchmarking for private blockchain systems are very specific to use-cases and are generally tied to a blockchain platform. In this article, we presentBlockMeter, an application agnostic performance benchmarking framework for private blockchain platforms. This framework can be utilised to measure the key performance matrices of any application deployed on top of an external private blockchain application in real-time. In this article, we present the architecture of the framework and discuss its different implementation aspects. Then, to showcase the applicability of the framework, we use BlockMeter to evaluate the two most widely used Hyperledger platforms, Hyperledger Fabric and HyperledgerSawtooth, against a number of use-cases.

==> protocol.tex <==
\section{Implementation and Protocol Flow}
\label{sec_implementation}
Based on the architecture of the framework, we have developed a Proof of Concept (PoC) in order to evaluate its applicability. In this section, we discuss how we have implemented the PoC and present the protocol flow which illustrates how different components of the architecture interact for a particular testing scenario. 


As illustrated in the architecture discussed earlier in section \ref{sec_architec}, a framework has been developed as a PoC that can measure the performance matrices of two different blockchain platforms under the Hyperledger Umbrella Projects \cite{hyperledgersite}. 

\subsection{Implementation}
At the Blockchain Aplication level (Blockchain Application part of section \ref{sec_architec}), Hyperledger Fabric network consisting of various number of ordering service nodes and endorsing peers were configured. In case Sawtooth network, various number of validating nodes and transaction processor nodes were set up. For both cases, the blockchian application was deployed using AWS EC2 instances and Docker(used for virtualisation). The network topology and structure was varied for different experiments.
    
The Target SDK for Hyperledger Fabric are available in Golang, Java, Python, NodeJs, etc, while Hyperledger Sawtooth SDK are also available in python, NodeJs and Rust. We have used the NodeJs SDKs for our implementation to create a middleware (refer to Transaction Processor in section \ref{sec_architec}), which accepts complies client requests into platform specific objects that can communicate with the backend blockchain network using the SDK functions.

The Performance recorder is a server set up using NodeJs \cite{nodejs} and Express \cite{express}. The server was hosted on an AWS EC2 machine exposing two POST APIs. The requests were routed to the blockchain network at the backend using an in instance of the appropriate class. This server also facilitates transaction throughput monitoring which tracks the number transactions completing per second and resource monitoring which records the resource consumption of the peer nodes every three seconds (because each request for the docker statistics takes more than two seconds to respond).

Two API ends are exposed from the NodeJs-Express \cite{nodejs} \cite{express} server. Client application submits transaction requests to different routes/API based on different blockchain platform that in under test. The requst is converted into a transaction proposal and then submitted to the corresponding transaction handler which pre-processes the transaction and submits to the blockchain network and responds back with a success code once transaction is appended to the ledger successfully.

The Fabcar\cite{fabcar01} application from the Hyperledger Fabric repository was used as a Blockchain Application that performed simple ledger operations like create, read and update. In case of Sawtooth platform, we developed a transaction processor similar to the fabcar application, so that we can compare the results. Several network configurations consisting of single and multiple ordering and validating nodes where deployed using docker so as to identify the variation in performance.

% In the next section a description of the protocol flow between the different components of the framework is described.

\subsection{Protocol Flow}
\label{sec_methodology}
In order to portray a typical situation, HTTP requests consisting transaction particulars are generated from \textit{Apache JMeter} \cite{jmeter01} that fetches those parameters from a preloaded CSV file and submits them to the respective blockhain path at the \textit{API Gateway}. Once the transaction parameters are received at the \textit{Transactions Handler} an instance of the request is created and passed on for framing a transaction object to the \textit{Transaction Processor} that pre-processes the object and submit time is recorded simultaneously. Once pre-processed, the transaction is submitted to the blockchian for valiadation, endorsement and execution. 

In the next steps, upon receiving valid response finish time is recorded. The API is then notified of success status. In the mean time number of transactions processed per second, and resource usage by docker containers are also recorded by the \textit{Performance Monitor}. These steps are illustrated graphically in figure \ref{meth_image}. Finally, the \textit{Performance Data} consisting of transaction latency, transaction throughput and resource consumption are recorded in JSON format into the file system. The records are then normalized, reformatted and converted into tabular format using NodeJs and python libraries that can be examined for comprehension of the performance.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{images/proto.pdf}
    \vspace{-20mm}
    \caption{Protocol Flow}
    \label{meth_image}
    \hspace*{\fill}
    \vspace{0mm}  
\end{figure*}

==> tableBackup.tex <==
\centering
\begin{tabular}{l|l|c|c|c|c|c} 
\toprule
\multicolumn{2}{l|}{Related Work}                                                              & ~H. F. Leppelsack~ & Blockbench & S. Pongnumkul, et al.~ & P. Thakkar et al.~ & BlockMeter  \\ 
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Blockchain \\Platforms\end{tabular}} & Fabric & O \CIRCLE & O & O & O & O\\ \cline{2-7}
& Sawtooth  & X & X & X & X & O\\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Evaluation \\Tool\end{tabular}}      & PoC          & X                  & O          & X                      & X                  & O           \\ 
\cline{2-7}
                                                                                & Caliper      & O                  & X          & X                      & X                  & X           \\ 
\cline{2-7}
                                                                                & Other        & X                  & X          & O                      & O                  & X           \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Evaluation \\Matrices\end{tabular}}  & Latency      & O                  & O          & X                      & X                  & O           \\ 
\cline{2-7}
                                                                                & Throughput   & O                  & O          & O                      & O                  & O           \\ 
\cline{2-7}
                                                                                & Resource     & X                  & X          & O                      & O                  & O           \\ 
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Evaluation \\Criteria\end{tabular}}  & Read/Write   & O                  & O          & O                      & O                  & O           \\ 
\cline{2-7}
                                                                                & Data Heavy   & O                  & O          & X                      & X                  & O           \\ 
\cline{2-7}
                                                                                & CPU Heavy    & O                  & O          & X                      & X                  & O           \\ 
\cline{2-7}
                                                                                & Scalability  & X                  & X          & X                      & X                  & O           \\ 
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Testing \\Environment\end{tabular}}  & Web Service  & X                  & N/A        & O                      & X                  & O           \\ 
\cline{2-7}
                                                                                & Local Server & O                  & N/A        & X                      & O                  & X           \\
\bottomrule
\end{tabular}
